LASER: Tuning-Free LLM-Driven Attention Control for Efficient Text-conditioned Image-to-Animation

Revolutionary advancements in text-to-image models have unlocked new dimensions for sophisticated content creation, such as text-conditioned image editing, enabling the modification of existing images based on textual guidance. This capability allows for the generation of diverse images that convey highly complex visual concepts. However, existing methods primarily focus on generating new images from text-image pairs and struggle to produce fine-grained animations from existing images and textual guidance without fine-tuning. In this paper, we introduce LASER, a tuning-free LLM-driven attention control framework that follows a progressive process: LLM planning, feature-attention injection, and stable animation generation. LASER leverages a large language model (LLM) to refine general descriptions into fine-grained prompts, guiding pre-trained text-to-image models to generate aligned keyframes with subtle variations. The LLM also generates control signals for feature and attention injections, enabling seamless text-guided image morphing for various transformations without additional fine-tuning. By using the same initial noise inversion from the input image, LASER receives LLM-controlled injections during denoising and leverages interpolated text embeddings to produce a series of coherent animation frames. We propose a Text-conditioned Image-to-Animation Benchmark to validate the effectiveness and efficacy of LASER. Extensive experiments demonstrate that LASER achieves impressive results in consistent and efficient animation generation, establishing it as a powerful tool for producing detailed animations and opening new avenues in digital content creation.

==> sec/3_method_beifen.tex <==
\section{Methodology}
\label{sec:method}

Given a user-defined descriptor \( P_* \) and an initial image \( I_0 \) (provided or generated), our method generates an animation sequence \(\{x_0^{(\alpha)}, x_1^{(\alpha)}, \ldots, x_n^{(\alpha)}\}\), where \(\alpha\) varies from 0 to 1. The length of the \( x_i^{(\alpha)} \) sequence is set by \( n_f \) and the number of sequences \( x_i^{(\alpha)} \) corresponds to the transformation stages \( n_t \). The resulting animation should retain the structure of $I_0$ while incorporating the characteristics described by \( P_* \).

\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{./figure/method.pdf}
\caption{Overview of proposed \method{}. (a) The LLM-driven Controller parses descriptive prompts to generate animation frame prompts. (b) It converts these prompts into control signals for texture and non-rigid editing. (c) The animation generator uses linear interpolation to ensure smooth transitions between keyframes, enabling fluid animation.
% the Starting with user input $P_*$ (and $I_0$), the LLM generates a series of descriptive prompts $\{P_0, P_1, \ldots, P_{n_{t}}\}$ for each key animation stage. 
% The initial prompt $P_0$ is utilized by the Stable Diffusion Prompt Generator Agent to generate the starting image $I_0$ (execute only when the user input consists solely of text), followed by DDIM Inversion to derive the latent noise $Z_{0T}$.
% This noise undergoes a denoising process to extract features and self-attention information, which are then used to reconstruct the image $x_0$ and following injection. For subsequent images like Keystage1 $x_1$, $Z_{0T}$ is duplicated to form $Z_{1T}^*$, which is then subjected to feature and self-attention injections specifically designed for processing by the U-Net, yielding $x_1$. The DDIM Inversion of $x_1$ gives rise to $Z_{1T}$, and together with $Z_{0T}$, they are linearly spherical interpolated to create the latent noise $Z_{T\alpha}^0$ for intermediate frames. This step, leveraging interpolated text embeddings $e_{\alpha}^0$ from prompts $P_0$ and $P_1$, enables the denoising U-Net to incorporate feature and self-attention injections, thus generating the intermediate frames $x_0^{\alpha}$. This iterative process, guided by the LLM, is repeated for all subsequent stages, ensuring a coherent animation flow that seamlessly integrates texture and non-rigid transitions.
}
\label{fig:method}
\end{figure*}


\subsection{Preliminary for Diffusion Models}

Diffusion models~\cite{ho2020denoising, song2020denoising, nichol2021improved} are probabilistic generative models that generate images by gradual denoising a noise distribution, typically Gaussian noise. The process involves two phases: a \textit{forward} process that adds noise to data, and a \textit{reverse} process that removes noise to reconstruct the image. Starting from pure noise, the reverse process iteratively refines the image by predicting and subtracting noise, ultimately producing a clean image.



We use a text-conditioned Stable Diffusion (SD) model~\cite{rombach2022high} that operates in a lower-dimensional latent space instead of pixel space. Images are first encoded into latent representations by a variational auto-encoder (VAE)~\cite{kingma2013auto_dis5}, followed by diffusion-denoising within the latent space. The denoised latent representation is then decoded back into the image space to produce the final image.



In the noise-predicting network $\epsilon_{\theta}$, residual blocks generate intermediate features $f_t^{l}$, which are used in the self-attention module to produce $Q$, $K$, and $V$ for capturing long-range interactions. Cross-attention then integrates the textual prompt $P$, merging text and image semantics. The attention mechanism is formulated as:
\begin{equation}
    Attention(Q, K, V) = softmax(\frac{QK^T}{\sqrt{d_k}})V
\end{equation}
where $Q$, $K$, and $V$ represent queries, keys, and values, with $d_k$ denoting the key/query dimension. Attention layers in the SD model significantly influence image composition and synthesis, guiding editing by manipulating attention during denoising~\cite{hertz2022prompt, tumanyan2023plug}.




% \subsection{Aligning text prompt generation and text embedding interpolation}
\subsection{LLM-driven Controller} \label{prompt extractor}
% In this section, we utilize LLM to generate aligned textual prompts for generating keyframes of animation.
In this section, we employ an LLM to extract aligned textual prompts for each transformation stage, accommodating both text-image pairs and text-only inputs. If an image is provided, it serves as the initial image \(I_0\); otherwise, we utilize pre-trained Stable Diffusion models to generate \(I_0\). To produce animations that faithfully align with the specified text description \(P_*\), we generate a series of text prompts \(\{P_0, P_1, \ldots, P_{n_{t}}\}\) for each transformation stage.



To enhance the quality and stability of the process, we introduce three LLM-based agents: Stage Image Text Prompt Agent'' (SIA), Stable Diffusion Prompt Generator Agent'' (PGA), and ``Injection Control Agent'' (ICA). Each LLM agent performs specific functions using predefined system prompts, without requiring any fine-tuning.


\subsubsection{SIA.}
Initially, SIA generates text prompts that guide the image generation for each key animation stage, as illustrated in Fig. \ref{fig:method} (a). The SIA generates text prompts based on two principles: 
i) By decomposing the animation descriptor \(P_*\) into independent processes, SIA reduces semantic differences between prompts, enhancing overall quality. For instance, the phrase ``A year has passed on the spring meadow.'' can be divided into four prompts: ``The meadow in spring.'', ``The meadow in summer.'', ``The meadow in autumn.'', and ``The meadow in winter.''. 
ii) Prompts must be highly aligned to ensure high-quality intermediate results through linear interpolation. Consistent sentence structures, such as ``A cat [\texttt{action}] on the ground'' and ``A [\texttt{animal}] jumping on the ground,'' minimize the gap between adjacent embeddings in the CLIP text embedding space \cite{kawar2023imagic}.

\subsubsection{PGA.} 
When user input lacks an image, PGA transforms broad concepts from the SIA into detailed prompts, guiding the Stable Diffusion model to generate $I_0$. As illustrated in Fig. \ref{fig:method} (a), PGA refines the initial text prompt from SIA by incorporating specific elements like texture, lighting, and artistic style, thereby creating a more detailed description. This enhancement enables Stable Diffusion to produce images of higher fidelity and complexity~\cite{lian2024llmgrounded}.


\subsubsection{ICA.} 
To generate diverse animations, we utilize a range of feature and attention injection strategies.  To select the appropriate strategy tailored to the animation type, we introduce the ICA, which determines the injection strategy during animation frame generation, based on inputs from the SIA.



% After generating the text prompts corresponding to each key stage ${P_0, P_1, \ldots, P_n}$, we obtain the respective text embeddings ${e_0, e_1, \ldots, e_n}$. When generating intermediate images, we perform a simple linear interpolation between the text embeddings of two adjacent key stages to obtain the corresponding text embedding $e$.

% \begin{equation}
% e_{\alpha}^{i} = (1 - \alpha)e_i + \alpha e_{i+1}
% \end{equation}

% In the construction of the animation sequence, the interpolation parameter \( \alpha \) is discretized into a series of values that facilitate a smooth transition between frames. This discretization is achieved by defining a set of equidistant points within the closed interval \([0, 1]\), where the number of points corresponds to the intended number of frames in an animation stage, denoted as $n_f$. Thus, \( \alpha \) takes on values \( \alpha_0, \alpha_1, \ldots, \alpha_{n_{f}-1} \), where \( \alpha_0 = 0 \) signifies the starting frame, and \( \alpha_{n_{f}-1} = 1 \).
%  corresponds to the ending frame, and intermediate values of \( \alpha \) represent proportionally spaced frames within the animation sequence. This linear spacing ensures that each frame is a weighted blend of the preceding and following key stage embeddings, rendering a gradual and continuous transformation throughout the animation.



\subsection{LLM-controlled Injection}
After receiving text prompts \(\{P_0, P_1, \ldots, P_{n_{t}}\}\), the model will sequentially generate the animation sequence \(\{x_0^{(\alpha)}, x_1^{(\alpha)}, \ldots, x_n^{(\alpha)}\}\), where $n$ = $n_t-1$. The animation $x_i^{(\alpha)}$ will depict the transition from $P_i$ to $P_{i+1}$. To maintain a certain structure in the images, the initial noise for each animation frame is obtained through performing DDIM Inversion on the last frame $x^1_{i-1}$ of the previous animation (with the first animation using the input image $I_0$). For a single animation frame $x_i^{\alpha}$, its initial noise $z_T^{i*}$ is copied from $z_T^i$. We then perform a simple linear interpolation between the text embeddings of two adjacent key animation stages to obtain the corresponding text embedding:

\begin{equation}
e_{i}^{\alpha} = (1 - \alpha)\cdot e_i + \alpha \cdot e_{i+1}
\end{equation}
where $e^i$ and $e^{i+1}$ are the text embeddings corresponding to $P_i$ and $P_{i+1}$, respectively. The interpolation parameter $\alpha$ is discretized into a series of equidistant values within the interval $[0, 1]$ to facilitate a meaningful transition between frames. The number of discrete values corresponds to the intended number of frames, denoted as $n_f$. Thus, $\alpha$ takes on values $\alpha_0, \alpha_1, \ldots, \alpha_{n_f-1}$, where $\alpha_0 = 0$ represents the starting frame and $\alpha_{n_f-1} = 1$ indicates the ending frame. This linear spacing ensures a continuous transformation across the animation sequence as shown in Fig.~\ref{fig:inter}.


\begin{figure}[t]
\centering
\includegraphics[width=0.98\linewidth]{./figure/inter.pdf}
\caption{By leveraging interpolation of text embeddings, meaningful intermediate images can be generated. }
\label{fig:inter}
\end{figure}



However, directly applying the vanilla DDIM process fails to produce desired animation, particularly when the input image is of anime style, a domain at which Stable Diffusion is less proficient. As shown in Fig. \ref{fig:ablation_method} (d), this approach not only fails to align the first frame with the input image but also loses the structural integrity of the input image in subsequent frames, leading to an unsatisfactory result.


\begin{figure}[t]
\centering
\includegraphics[width=0.98\linewidth]{./figure/ablation_method.pdf}
\caption{Overview of Feature and Association Injection. }
\label{fig:ablation_method}
\end{figure}


\subsubsection{Texture Transformation.}

To address texture changes, we propose an LLM-controlled feature and attention injection approach. Specifically, we first perform DDIM Inversion on the prior image $I_0$ or $x_{i-1}^1$ to extract residual block features $f_t^i$ and self-attention projections $q_t^i$, $k_t^i$, and $v_t^i$, ultimately obtaining the initial latent representation $z_T^i$. Our method, termed "Feature and Association Injection" (FAI), injects selected features $f_{t-1}^i$ into the fourth layer of residual blocks, while propagating self-attention elements $q_{t-1}^i$ and $k_{t-1}^i$ across decoder layers, as illustrated in Fig.~\ref{fig:Injection}.
During the denoising process at each frame, we perform a two-step interpolation on the value components. First, we interpolate between the values from the first and last frames based on the current frame index weight $a_i$. Then, we further blend this intermediate result with the current value component using a time-step decay weight $\lambda = \frac{t}{T}$, formulated as:

\begin{equation}
v_{t}^{i**} = (1-\gamma) \cdot (\alpha \cdot v_{t}^{0*} + (1-\alpha) \cdot v_{t}^{1*}) + \gamma \cdot v_{t}^{i*}  
\end{equation}

The extracted $q$, $k$, and $f$ from the source image effectively preserve structural consistency across animation frames~\cite{tumanyan2023plug}, while the progressive interpolation of $v$ ensures smooth texture transitions, as depicted in Fig.~\ref{fig:ablation_method}~(c).







\subsubsection{Enhancing Generation Quality}

With FAI, animation frame quality improves significantly over vanilla DDIM, but issues remain: (i) the first frame misaligns with the input image, (ii) frames lose detail, and (iii) weak prompt adherence. While classifier-free guidance (CFG) enhances text conditioning, it struggles with guidance scales over 1.0. To address this, we replace the null-text embedding with the input text prompt embedding $e_i$ for frame $x_i^{\alpha}$, as shown in Fig.~\ref{fig:ablation_method}(b). This preserves the input image’s structure while enabling prompt-driven edits~\cite{miyake2023negativepromptinversionfastimage}, resulting in detailed, coherent frames that align with both the input image and textual guidance, as shown in Fig.~\ref{fig:ablation_method}(a).



\begin{figure}[t]
\centering
\includegraphics[width=0.98\linewidth]{./figure/Injection.pdf}
\caption{Overview of our injection methods. }
\label{fig:Injection}
\end{figure}


\subsubsection{Non-Rigid Transformation.} 
%Nevertheless, the aforementioned method struggles with non-rigid modifications. The typical solution—limiting injection range to rigid changes—risks losing image identity. To address this, especially for non-rigid edits, we avoid injecting into residual blocks to preserve the image's structure. Instead, we use targeted attention injections. Since image layout solidifies early in denoising and self-attention queries align semantically~\cite{cao2023masactrl}, they can extract content from various objects. After a specific timestep, we inject keys $k_{t-1}^i$ and values $v_{t-1}^i$ from the previous inversion stage, as shown in Fig. \ref{fig:Injection}. This forms object outlines from text prompts and enriches structure with details from the source image, enabling semantically coherent images that support non-rigid transitions. We refer to this as ``Key-Value Attention Injection'' (KVAI).

While effective, the previous method struggles with non-rigid modifications. To address this, we avoid injecting into residual blocks to preserve image structure and instead apply targeted attention injections. Since image layout stabilizes early in denoising and self-attention queries align semantically~\cite{cao2023masactrl}, they can effectively extract content from various objects. At a specific timestep, we inject keys $k_{t-1}^i$ and values $v_{t-1}^i$ from the inversion stage.
To ensure smooth structural transitions, we linearly interpolate the query between the first and last frames using the current frame weight $a_i$ and further blend it with the corresponding value via time-step decay interpolation, formulated as:

\begin{equation}
k_{t}^{i**} = (1-\gamma) \cdot (\alpha \cdot k_{t}^{0*} + (1-\alpha) \cdot k_{t}^{1*}) + \gamma \cdot k_{t}^{i*}  
\end{equation}

Additionally, we incorporate cross-frame attention during injection, enabling each frame’s query $q$ to access all frames’ keys and values. This enhances structural consistency, refines object outlines from text prompts, and enriches frames with source image details, facilitating semantically coherent non-rigid transitions. We refer to this approach as **Key-Value Attention Injection (KVAI)**, as illustrated in Fig.~\ref{fig:Injection}.








\subsubsection{Hybrid Transformation.}
Additionally, we introduce **Decremental Key-Value Attention Injection** (DAI) to generate animation sequences that integrate both texture changes and non-rigid transformations, as illustrated in Fig.~\ref{fig:Injection}. In this approach, the animation undergoes a complete non-rigid transformation from start to end, while textures evolve progressively under prompt guidance, ultimately retaining only partial features from the input image. Similar to KVAI, DAI follows a comparable processing framework, with the key distinction that it interpolates between $k_{t-1}^i, v_{t-1}^i$ and $k_{t}^{i*}, v_{t}^{i*}$ to obtain $k_{t}^{i**}, v_{t}^{i**}$. This interpolation enables smoother transitions between frames, ensuring coherent integration of both texture and structural transformations. Furthermore, we incorporate **cross-frame attention** during injection to enhance frame consistency, further improving the overall temporal coherence of the animation.



\begin{equation}
k_{t}^{i**} = (1 - \beta)k_{t-1}^i + \beta k_{t}^{i*}, \\
v_{t}^{i**} = (1 - \beta) v_{t-1}^i + \beta v_{t}^{i*},
\end{equation}
where \(\beta = w * \alpha\), \(w \in (0, 1)\). In text embedding interpolation, \(\beta\) can replace \(\alpha\) to achieve a higher-quality final frame. This mechanism ensures a gradual and smooth transition in the hybrid transformation process. The layers and timesteps utilized in DAI are the same as those in KVAI.

\subsubsection{More details on ICA.} 
we develop the ICA to select the optimal injection strategy at each stage of animation generation, as shown in Fig. \ref{fig:method} (a). We set a specific system prompt for LLM to build ICA, which can determine the type of change, process inputs from SIA, and output corresponding signals to the model, guiding specific output behaviours. By precisely managing attention injection at each stage, ICA ensures that the generated animations are visually coherent and align closely with the textual descriptors. ICA analyzes inputs from SIA, assesses differences between adjacent text prompts, and instructs the model to apply the appropriate injection strategy when generating animation frames.


\subsection{Animation Generator} 
To create the sequence $x_i^{(\alpha)}$, comprising a series of animation frames $x_i^{\alpha}$, we start by deriving the text embeddings $e_{\alpha}$ through interpolation between $e_i$ and $e_{i+1}$. 
Subsequently, the latent variable $z_T^{i*}$ undergoes denoising, during this phase, it is subjected to feature and attention injections governed by the ICA, ultimately producing 
$x_i^{\alpha}$. 
The first frame, denoted by  $\alpha = 0$, precisely reconstructs the input image.
As $\alpha$ progresses from 0 to 1, the influence of $P_i$ gradually decreases,  whereas the influence of $P_{i+1}$ correspondingly escalates.
The sequence $x_i^{(\alpha)}$ is completed with the generation of the final frame $x_i^1$.
If $P_{i+2}$ is available, the model performs DDIM Inversion on $x_i^1$ to obtain a new initial noise $z^{i+1}_T$, and the process is repeated.







==> sec/7_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/8_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
